Towards Practical Few-shot Federated NLP

Transformer-based pre-trained models have emerged as the predominant solution for natural language processing (NLP). Fine-tuning such pre-trained models for downstream tasks often requires a considerable amount of labeled private data. In practice, private data is often distributed across heterogeneous mobile devices and may be prohibited from being uploaded. Moreover, well-curated labeled data is often scarce, presenting an additional challenge. To address these challenges, we first introduce a data generator for federated few-shot learning tasks, which encompasses the quantity and skewness of scarce labeled data in a realistic setting. Subsequently, we propose AUG-FedPrompt, a prompt-based federated learning system that exploits abundant unlabeled data for data augmentation. Our experiments indicate that AUG-FedPrompt can perform on par with full-set fine-tuning with a limited amount of labeled data. However, such competitive performance comes at a significant system cost.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> alg-trial.tex <==
\begin{algorithm}
	\footnotesize
	\SetAlgoNoEnd
  \SetKwProg{Fn}{Function}{~}{end}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{MIN}{MIN}\SetKwFunction{MAX}{MAX}\SetKwFunction{LENGTH}{LENGTH}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Variable}{Variable}

  \Input{
      % Pre-trained model, $\Theta$;\\
      Model capacity threshold, $\varphi $;\\
      Trial interval, $trial\_intvl$;\\
      Start-up depth and width, $D_{0}$ and $W_{0}$;\\
      Step of depth and width, $S_d$ and $S_w$.
    }

  \Output{
      Fine-tuned adapter weights, $\Theta_{i}$~(i=1,2\dots).
      % $Q_b$\;   
    }
  \BlankLine

  \Fn{Cloud\_controller():}{
    $Trial_{0}$, $Trial_{1}$, $Trial_{2}$ $\leftarrow$ selects $3N$ clients;\\
    Iteration i=0;\\
    $T_{trial}$=$T_{now}$;\\
    Dispatch(0); // Init model and trigger client training\\
      \While{Eval() $<$ $acc$}
      { 
        i++;\\
        $\Theta^{k}_{i}(n)$ $\leftarrow$ Receive updated adapters from $Trial_{k}$;\\
      $\Theta^{k}_{i}$ $\leftarrow$ Fedavg($\Theta^{k}_{i}(n)$);\\
      $Trial_{0}$, $Trial_{1}$, $Trial_{2}$ $\leftarrow$ selects $3N$ new clients;\\
        \eIf{$T_{now}$ - $T_{trial}$ > $trial\_intvl$}{Compare accuracy under different $\Theta^{k}_{i}$;\\
        $\Theta_{i}$ $\leftarrow$ Winner track;
        $D_{i}, W_{i}$ $\leftarrow$ Winner setting;\\
        $T_{trial}$=$T_{now}$;\\
        Dispatch(i) // Inherit winner track;\\}{
          Send the aggregated model $\Theta^{k}_{i}$ to $Trial_{k}$.
        }
      }
      Exit training.
    }

  \Fn{Client\_training(i,k):}{
    $\Theta_{i}^{k}$ $\leftarrow$ Receive global adapter  from cloud;\\
    $\Theta_{i+1}^{k}(n)$ $\leftarrow$ Train and update local adapter; \\
    Send updated adapter $\Theta_{i+1}^{k}(n)$ to cloud.
  }
  
  \Fn{Dispatch(i):}{
    $F$($D$,$W$): Initial/Inherit winner track $\Theta_{i}$ with $D$, $W$.
  
  $\Theta_{i}^{0}$ $\leftarrow$ $F$($D_{i}$,$W_{i}$);
  $\Theta_{i}^{1}$ $\leftarrow$ $F$($D_{i}+S_{d}$,$W_{i}$);
  $\Theta_{i}^{2}$ $\leftarrow$ $F$($D_{i}$,$W_{i}+S_{w}$);\\
  Sends $\Theta_{i}^{0}$, $\Theta_{i}^{1}$, $\Theta_{i}^{2}$ to $Trial_{0}$, $Trial_{1}$, $Trial_{2}$ seperately\;
  Parallel: Client\_training(i,k).
  }
  
  \caption{Cross-device Soft Label Annotating}\label{alg:soft-label}
\end{algorithm}


==> fig-def-distribution.tex <==
\begin{figure*}[t]
	\centering
        \includegraphics[width=0.6\textwidth]{figs/def-distribution.pdf}

	%  \vspace{-10pt}
	\caption{We define a new triple tuple (samples, clients, sparsity): noted as ($n$, $\xi$, $\gamma$) to represent the true few show learning (labeled) data distribution. \mwx{N-ways K-shots: way means number of labels, shot means data quantity for each label.}} 
	% \vspace{-15pt}
	\label{fig:def-distribution}
\end{figure*}

==> fig-def-fednlp-beta.tex <==
\begin{figure}[t]
	\centering
	 \includegraphics[width=0.45\textwidth]{figs/def-fednlp-beta.pdf}
	%  \vspace{-10pt}
	\caption{The probability density of quantity of training examples in each of the 100 clients on the 20News dataset with different $\beta$. When $\beta$ is larger, then all clients share more similar numbers of examples; when $\beta$ is smaller, then the range of the quantity is much wider — i.e., the larger differences between clients in terms of their sizes of datasets.} 
	% \vspace{-15pt}
	\label{fig:def-fednlp-beta}
\end{figure}

==> fig-def-fsl-distribution.tex <==
\begin{figure}[t]
	\centering
	 \includegraphics[width=0.45\textwidth]{figs/def-fsl-distribution.pdf}
	%  \vspace{-10pt}
	\caption{Different data distribution for FSL. \mwx{Should be replaced by a system design picture or system implementation comple workflow (including cloud pre-training, labeled data input and fine-tuning on mobile devices.).}} 
	% \vspace{-15pt}
	\label{fig:def-fsl-distribution}
\end{figure}

% \begin{figure}[t]
% 	\centering
% 	 \includegraphics[width=0.27\textwidth]{figs/design-adapter-arch.pdf}
% 	 \vspace{-5pt}
% 	\caption{The structure of adapters used.} 
% 	\vspace{-10pt}
% 	\label{fig:design-adapter-arch}
% \end{figure}


==> fig-eval-augmentation.tex <==
\begin{figure}[t]
	\centering

    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=0.98\textwidth]{figs/eval-augmentation-agnews.pdf}
        \subcaption{AGNEWS}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=0.98\textwidth]{figs/eval-augmentation-agnews.pdf}
        \subcaption{Dataset 2}
    \end{minipage}
	%  \vspace{-10pt}
	\caption{Using unlabeled data for augmentation via soft label inferring.} 
	% \vspace{-15pt}
	\label{fig:def-eval-augmentation}
\end{figure}

==> fig-eval-gain-gap.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}[b]{1\textwidth}
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_agnews_roberta-large.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_mnli_roberta-large.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yelp-full_roberta-large.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yahoo_roberta-large.pdf}
        \end{minipage}
    \end{minipage}
    \subcaption{Roberta-Large \mwx{datapoints for Usable accuray instead of fixed 0.1\%.}}
    
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_agnews_roberta-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_mnli_roberta-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yelp-full_roberta-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yahoo_roberta-base.pdf}
        \end{minipage}
    \end{minipage}
    \subcaption{(Roberta-Base)}

    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_agnews_bert-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_mnli_bert-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yelp-full_bert-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yahoo_bert-base.pdf}
        \end{minipage}
    \end{minipage}
    \subcaption{(BERT-Base)}

    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_agnews_albert-base-v2.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_mnli_albert-base-v2.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yelp-full_albert-base-v2.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yahoo_albert-base-v2.pdf}
        \end{minipage}
    \end{minipage}
    \subcaption{(ALBERT-BASE-V2)}
\end{minipage}
    \caption{Time-to-accuracy throughout a training session. FedPrompt speeds up model convergence significantly. Model is BERT. Sample data: 40. \mwx{cut x-axis to 100 iters}}    \label{fig:eval-gain-gap}
%    \caption{The time-to-accuracy of \sys and baselines with base BERT model.}
    % \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
    
\end{figure*}

% \begin{table*}[]
%     \footnotesize
%     \begin{tabular}{|l|ll|ll|ll|ll|}
%     \hline
%              & \multicolumn{2}{c|}{TC (20news)}    & \multicolumn{2}{c|}{TC (agnews)}   & \multicolumn{2}{c|}{TC (semeval)}   & \multicolumn{2}{c|}{ST (onto)}       \\ \hline
%     Methods & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup \\ \hline
%     Origin   & \multicolumn{1}{l|}{26.70} & 1      & \multicolumn{1}{l|}{44.49} & 1.00  & \multicolumn{1}{l|}{260.67} & 1.00  & \multicolumn{1}{l|}{1034.31} & 1.00  \\ \hline
%     Freeze   & \multicolumn{1}{l|}{7.10}  & 3.76   & \multicolumn{1}{l|}{14.02} & 3.17  & \multicolumn{1}{l|}{105.39} & 2.47  & \multicolumn{1}{l|}{649.47}  & 1.59  \\ \hline
%     Adaptive & \multicolumn{1}{l|}{0.18}  & 150.40 & \multicolumn{1}{l|}{0.67}  & 66.78 & \multicolumn{1}{l|}{2.63}   & 99.13 & \multicolumn{1}{l|}{33.60}   & 30.78 \\ \hline
%     \end{tabular}
%     \caption{Network Traffic Save}
%     \label{tab:eval-communication}
%     \end{table*}

==> fig-eval-local-fsl.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.3\textwidth}
        \includegraphics[width=0.98\textwidth]{figs/eval-local-fsl-performance.pdf}
        \subcaption{Performance}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.2\textwidth}
        \includegraphics[width=0.98\textwidth]{figs/eval-local-fsl-distribution.pdf}
        \subcaption{Distribution}
    \end{minipage}
    \caption{Local prompt learning performance. (a) N sample(s) per client; (b) Different samples per client performance after 1 iteration training. Local epoch is 10, Clients in total is 10, dataset is AGNEWS, Model is BETR, Train bs is 4.}
    \label{fig:eval-local-fsl}
\end{figure}

==> fig-eval-performance-gain.tex <==
% \begin{figure}[t]
% 	\centering
%     \begin{minipage}[b]{0.23\textwidth}
%         \includegraphics[width=0.98\textwidth]{figs/eval-performance-gain.pdf}
%         \subcaption{AGNEWS}
%     \end{minipage}
%     ~
%     \begin{minipage}[b]{0.23\textwidth}
%         \includegraphics[width=0.98\textwidth]{figs/eval-performance-gain.pdf}
%         \subcaption{Dataset 2}
%     \end{minipage}
% 	%  \vspace{-10pt}
% 	\caption{Accuracy gain turns more obvious when labeled data is extremely few.} 
% 	% \vspace{-15pt}
% 	\label{fig:def-eval-performance-gain}
% \end{figure}

\begin{figure}[t]
	\centering
        \includegraphics[width=0.3\textwidth]{figs/eval-performance-gain.pdf}

	%  \vspace{-10pt}
	\caption{The conclusion of Figure~\ref{fig:eval-performance-overall}. Accuracy gain turns more obvious when labeled data reaching the `balance point'. Y-axis=Pet-CLS} 
	% \vspace{-15pt}
	\label{fig:eval-performance-gain}
\end{figure}

==> fig-eval-performance-overall.tex <==
\begin{figure*}[t]
	\centering
        \includegraphics[width=0.8\textwidth]{figs/eval-performance-overall.pdf}

	%  \vspace{-10pt}
	\caption{Balance point is different for various datasets. \mwx{Can be moved to appendix.}} 
	% \vspace{-15pt}
	\label{fig:eval-performance-overall}
\end{figure*}

==> fig-eval-performance.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-performance-agnews.pdf}
            \subcaption{\texttt{AGNEWS}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-performance-mnli_40.pdf}
            \subcaption{\texttt{MNLI}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-performance-yelp-full_40.pdf}
            \subcaption{\texttt{YELP-F}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-performance-yahoo_40.pdf}
            \subcaption{\texttt{YAHOO}}
        \end{minipage}
    \end{minipage}
    
    
    \caption{Time-to-accuracy throughout a training session. FedPrompt speeds up model convergence significantly. Model is BERT. Sample data: 40.}    \label{fig:eval-performance-bert}
%    \caption{The time-to-accuracy of \sys and baselines with base BERT model.}
    % \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
    
\end{figure*}

% \begin{table*}[]
%     \footnotesize
%     \begin{tabular}{|l|ll|ll|ll|ll|}
%     \hline
%              & \multicolumn{2}{c|}{TC (20news)}    & \multicolumn{2}{c|}{TC (agnews)}   & \multicolumn{2}{c|}{TC (semeval)}   & \multicolumn{2}{c|}{ST (onto)}       \\ \hline
%     Methods & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup \\ \hline
%     Origin   & \multicolumn{1}{l|}{26.70} & 1      & \multicolumn{1}{l|}{44.49} & 1.00  & \multicolumn{1}{l|}{260.67} & 1.00  & \multicolumn{1}{l|}{1034.31} & 1.00  \\ \hline
%     Freeze   & \multicolumn{1}{l|}{7.10}  & 3.76   & \multicolumn{1}{l|}{14.02} & 3.17  & \multicolumn{1}{l|}{105.39} & 2.47  & \multicolumn{1}{l|}{649.47}  & 1.59  \\ \hline
%     Adaptive & \multicolumn{1}{l|}{0.18}  & 150.40 & \multicolumn{1}{l|}{0.67}  & 66.78 & \multicolumn{1}{l|}{2.63}   & 99.13 & \multicolumn{1}{l|}{33.60}   & 30.78 \\ \hline
%     \end{tabular}
%     \caption{Network Traffic Save}
%     \label{tab:eval-communication}
%     \end{table*}

==> fig-eval-sparsity.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-sparsity-gamma-fedpet-yahoo.pdf}
            \subcaption{\texttt{YAHOO} (non-iid)}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-sparsity-yahoo-alpha-0-seed-42-pattern-0.pdf}
            \subcaption{\texttt{YAHOO} (iid)}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-sparsity-gamma-fedpet-agnews.pdf}
            \subcaption{\texttt{AGNEWS} (non-iid)}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-heatmap-fedpet-mnli.pdf}
            \subcaption{\texttt{MNLI} (non-iid)}
        \end{minipage}
    \end{minipage}
    
    \caption{(a). Scattered is better under non-iid distribution; (b). More data brings benefit; (c). new dataset; (d) impact of clients. \mwx{maybe just show fewer gamma case. It would be looking better.}}    
    \label{fig:eval-sparsity}
    
\end{figure*}


==> rebuttal.tex <==
\section*{A. Common Question}
\subsection*{A1. Techniques of limited interest (\#3/\#4)}
This manuscript focus on the transformer-based NLP tasks.
In recent, many transformer-based models are proposed to boost the performance of enormous fields.
Our core designs, which target unleashing the full potential of pre-trained transformers, could be applied to other tasks, such as speech recognition~\cite{baevski2020wav2vec}, computer vision~\cite{liu2021swin}, and so on.
For example, wav2vec~\cite{baevski2020wav2vec} utilizes transformers to extract contextualized representations from acoustic waves.
It outperforms the previous state of the art on the 100-hour subset while using 100 times less labeled data.
Our techniques could be transferred to those tasks in order to enhance their few-shot performance under federated learning.

\section*{B. Individual Questions}
\subsection*{B1. Part of solution seems to be rather heuristic. (\#3)}
We admit the proposed filtering mechanism can easily be misinterpreted as being only heuristic due to the lack of in-depth description.
However, our filtering mechanism has been carefully designed and implemented to help filter out those wrong samples and remain the purity of augment dataset.
Details and more description could be found in our open-sourced code repository \url{https://github.com/caidongqi/AUG-FedPrompt}.


\subsection*{B2. Comparison of only with vanilla federated fine-tuning. (\#3)}
We add some ablation experiments in Table~\ref{tab:eval-softlabel-new} to show the necessity of orchestrating prompt and pseudo label.
AUG-FedPrompt achieves 85.8\%-97.0\% relative convergence accuracy to the full-set fine-tuning that assumes all data samples are labeled. 
Neither pseudo labeling nor prompt learning alone is enough to exhibit a usable accuracy. 
With only one of them, the relative convergence accuracy is 40\%-74\%.

\subsection*{B3. Lack of novelty. (\#4)}
We admit pseudo labeling is a common trick for machine learning training.
However, our technique contribution is composed of three parts: prompt, pseudo labeling, and their orchestrating.

Apart from introducing pseudo label, we are the first to apply discrete prompt to federated learning in order to boost the federated few-shot learning performance.
We avoid using `FedPrompt' because \cite{fedprompt} claims it before, but they use continuous prompt for parameter-efficient tuning, which is totally different from ours.

For the orchestrating of prompt and pseudo label, we find that pseudo labeling heavily relies on the initial model accuracy to get enough correct labels, for which prompt learning can help; 
in turn, prompt learning's ability is limited to the
few number of data labels, for which pseudo labeling can help.
The necessity of orchestrating them both is shown in Table~\ref{tab:eval-softlabel-new}.

\subsection*{B4. Confusing notation and the description. (\#4)}
We use $T$ and $T^{*}$ to differentiate a single token and multiple tokens.
$T$ is a single token for each output label, which represents its task-specific meaning in the pattern;
$\_\_ \in T$ is a mask token;
$T^{*}$ is the set of all token sequences for input text, which represents cloze questions containing a single mask.

The brick in the middle of Fig. 3 means training data and model.
More specifically, blue brick means text input; green brick means labels; yellow brick means pre-trained model; orange brick means fine-tuned model.
The colors are carefully chosen to match the workflow of local prompt training in the bottom half of the figure.
We should associate them more explicitly.

At last, we thank all the reviewers for their valuable reviews and hope our response could answer those questions.

\input{tab-eval-softlabel-new.tex}

==> sec-cost-energy.tex <==
\subsection{Energy consumption.}\label{sec:cost-energy}

==> sec-cost-memory.tex <==
\subsection{System Cost}\label{sec:cost}

==> sec-cost-network.tex <==
\subsection{Memory footprint.}\label{sec:cost-memory}

==> sec-eval-augmentation.tex <==
\subsection{Unlabeled Data Usage} \label{sec:eval-augmentation}

\input{fig-eval-augmentation.tex}

Simply augmenting training dataset via unlabeled data inferring does not bring benefit at all. But \textbf{FedPrompt with limited labeled data still lags behind full data fine-tuning.} That means unlabeled data has numerous potential for digging.

\textbf{Draw a line plot to show the margin between few shot Fedpet training and full dataset finetuning.}

Future work:
(1) How many unlabeled examples are tagged correctly?
(2) Assuming that all unlabeled examples are tagged correctly, how many benefit will be brought?

==> sec-eval-cost.tex <==
\subsection{System Cost}


Performance of various models, shown in Figure~\ref{fig:eval-model}.

\mwx{Expected conclusion:} Large-scale foundation model is needed to take full advantage of prompt learning. 

\mwx{Show the runtime that arriving the 90\% of full-set accuracy.} Instead of the runtime line because the accuracy gap will confuse the reviewers.

Mobile device: Jetson TX2.

Latency and peak memory of different foundation models.

\mwx{Eval the impact of models.}
BERT: some datasets perform bad. But whether it can caused by the origin BERT feature instead of FedPET.
That is to say, those dataset perform bad on BERT even fine-tuned on full dataset.



MobileBERT, DistilBERT, etc.
\begin{itemize}
    \item Energy exps: per-device energy consumption at average till convergence (bar plot).
    
    \item Network exps: per-device network cost at average till convergence (bar plot).
    
    \item Memory exps.
\end{itemize}





==> sec-eval-gain-gap.tex <==
% \subsection{Gain and Gap}  \label{sec:eval-gain-gap}

% \mwx{Will be merged to Section $\S$\ref{sec:eval-performance}}

% \textbf{Prompt learning performs better than vanilla fine-tuning.} Uniform few show learning results have been shown in Figure~\ref{fig:eval-gain-gap}.

% \input{tab-eval-todo.tex}

==> sec-eval-local-fsl.tex <==
\subsection{Local Prompt Learning Performance}

\input{fig-eval-local-fsl.tex}
Few examples can make such a big diff. There are there possible reasons:
1. learning rate is too large, some clients are witnessing overfitting 
2. local training epoch is too big, now it is 10 epochs before aggregation
3. pre-trained models maybe has ``data affinity". Clients owing data prefered by pre-trained models tend to achieve better accuracy. In addition, some data has better quality than others~\mwx{ref}.



==> sec-eval-prompt-tuning.tex <==
\subsection{Efficiency of Prompt Tuning} \label{sec:eval-pt}
Prompt tuning claims no more manual searching for hand-make prompt~\cite{lester2021power, liu2021p}. 
And further research shows its great performance on big models~\cite{liu2021gpt}.

First, hyper-parameter space is extremely large for training SOTA prompt tuning. 
It is a hard work to reproduce those excellent results. 
And most of them do not release their trained models~\cite{gu2021ppt}.

Second, even assuming that we are well knowledged with perfect hyper-parameter, it still need more iterations to converge compared to vanilla fine-tuning.
Fine-tuning of prompt embeddings requires even more steps~\cite{liu2021gpt}.
And they could only perform on par with vanilla fed fine-tune instead of outperforming (which we did through hard pt).

\mwx{What's the difference between ~\cite{lester2021power, liu2021p, liu2021gpt}?}

==> sec-related-pl.tex <==
\subsection{System Model} \label{sec:related-pl}
Prompt learning is first proposed by~\toref. It includes two mainstreams: hard prompt learning (a.k.a discrete prompt learning) and soft prompt learning (a.k.a continuous prompt learning).

\textbf{Hard prompt learning.}

\textbf{Soft prompt learning.}

Homogenization provides powerful leverage but demands caution, as the defects of the foundation model are inherited by all the adapted models downstream. 
Despite the impending widespread deployment of foundation models, we currently lack a clear understanding of how they work, when they fail, and what they are even capable of due to their emergent properties~\cite{bommasani2021opportunities}.

==> tab-eval-softlabel-new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|ccccc}
    \toprule
    \textbf{Dataset}       &  \begin{tabular}[c]{@{}c@{}}\textbf{Full-set}\\ \textbf{(oracle)}\end{tabular} &
    \begin{tabular}[c]{@{}c@{}}\textbf{Vanilla-}\\ \textbf{FedCLS}\end{tabular} &
    \begin{tabular}[c]{@{}c@{}}\textbf{Prompt-}\\ \textbf{Only}\end{tabular} &
    \begin{tabular}[c]{@{}c@{}}\textbf{Pseudo-}\\ \textbf{Only}\end{tabular} &
    \begin{tabular}[c]{@{}c@{}}\textbf{Both}\\ \textbf{(Ours)}\end{tabular} \\ 
    \midrule
    \texttt{AGNEWS} (skewed) & 93.0     & 64.8$\pm$3.1           & 68.4$\pm$2.4           & 67.5$\pm$1.3        & \textbf{90.2}$\pm$0.5    \\
    \texttt{MNLI} (skewed)   & 85.0     & 37.7$\pm$5.6          & 42.4$\pm$5.8           & 42.7$\pm$6.3           & \textbf{75.7}$\pm$1.2    \\
    \texttt{YAHOO} (skewed)  & 78.0     & 24.4$\pm$10.3           & 41.8$\pm$4.3           & 31.0$\pm$2.0           & \textbf{66.9}$\pm$1.1    \\
    \texttt{YELP-F} (skewed)   & 70.0     & 38.3$\pm$8.8           & 51.2$\pm$1.8           & 45.7$\pm$4.4           & \textbf{58.2}$\pm$2.4    \\\midrule
    \texttt{YELP-F} (uniform)  & 70.0        & 54.0$\pm$0.1           & 58.1$\pm$1.5         & 57.0$\pm$2.2           & \textbf{61.9}$\pm$0.7  \\
    \bottomrule
    \end{tabular}}
    \vspace*{-5pt}
    \caption{Convergence accuracy with 64 gold labels.
    ``Full-Set'' assumes every data is labeled (an oracle case).
    ``skewed'' means the gold labels are located on few clients instead of uniformly distributed across clients.}
    \label{tab:eval-softlabel-new}
    \vspace*{-10pt}
\end{table}

% \texttt{YELP} prompt: [0.57604, 0.60052, 0.56548]


% \begin{table}[t]
%     \centering
%     \scriptsize
%     \begin{tabular}{@{}cc|cccc@{}}
    
%     \toprule
%     \multicolumn{2}{c|}{Dataset}            & \texttt{AGNEWS} & \texttt{MNLI} & \texttt{YAHOO} & \texttt{YELP} \\ \midrule
%     \multirow{3}{*}{Uniform}& Full-set   & 93.0    & 85.0 & 78.0  & 70.0 \\ 
%                             &\texttt{FedCLS}   & 66.1$\pm$12.8    & 60.1$\pm$0.4 & 57.6$\pm$1.9  & 54.0$\pm$0.1 \\
%                             & FedPrompt     & \textbf{87.0}$\pm$0.8   & \textbf{77.6}$\pm$0.8 & \textbf{66.0}$\pm$0.1  & \textbf{61.9}$\pm$0.7 \\
%                             \midrule
%     \multirow{3}{*}{Skew}  &\texttt{FedCLS}   & 64.8$\pm$3.1   & 37.7$\pm$5.6 & 24.4$\pm$10.3  & 38.3$\pm$8.8 \\
%                             & FedPrompt     & 68.4$\pm$2.4   & 42.4$\pm$5.8 & 41.8$\pm$4.3  & 51.2$\pm$1.8 \\
%                             & w/ augment & \textbf{90.2}$\pm$0.5   & \textbf{75.7}$\pm$1.2 & \textbf{66.9}$\pm$1.1  & \textbf{58.2}$\pm$2.4 \\ \bottomrule
%     \end{tabular}
%     \caption{AUG-FedPrompt enhances performance under different few-shot learning settings. 
%     FedPrompt stands for AUG-FedPrompt without unlabeled data augmentation.
%     Datapoint: 64 for \texttt{AGNEWS}, 1024 for \texttt{MNLI}, 256 for \texttt{YAHOO} and \texttt{YELP}. }
%     \label{tab:eval-softlabel}
%     \vspace{-10pt}
% \end{table}

==> tab-eval-todo.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
    \begin{tabular}{llllll}
    \hline
    Examples                & Method & mnli          & agnews        & yahoo         & yelp          \\ \hline
    \multirow{2}{*}{T=40}   & FedCLS & 0.41          & 0.73          & 0.33          & 0.31          \\
                            & FedPET & \textbf{0.48} & \textbf{0.83} & \textbf{0.52} & \textbf{0.38}  \\ \hline
    \multirow{2}{*}{T=100}  & FedCLS & 0.45          & 0.81          & 0.50          & 0.41          \\
                            & FedPET & \textbf{0.48} & \textbf{0.87} & \textbf{0.65} & \textbf{0.43} \\ \hline
    \multirow{2}{*}{T=1000} & FedCLS & 0.54          & 0.89          & 0.65          & \textbf{0.53}     \\
                            & FedPET & \textbf{0.62} & \textbf{0.91} & \textbf{0.67} & 0.49          \\ \hline
    \end{tabular}
    \caption{\mwx{Comparison of different models.}
    Average accuracy and standard deviation for BERT on Yelp, AG's News, Yahoo and MNLI for four training set sizes $|\mathcal{T}|$. Model: BERT-base.}
    \label{tab:eval-todo}
    \end{table}
